Characterizing First Arrival Position Channels: Noise Distribution and Capacity Analysis

This paper introduces a novel mathematical model for Molecular Communication (MC) systems, utilizing First Arrival Position (FAP) as a fundamental mode of information transmission. We address two critical challenges: the characterization of FAP density and the establishment of capacity bounds for channels with vertically-drifted FAP. Our method relate macroscopic Partial Differential Equation (PDE) models to microscopic Stochastic Differential Equation (SDE) models, resulting in a precise expression that links FAP density with elliptic-type Green's function. This formula is distinguished by its wide applicability across any spatial dimensions, any drift directions, and various receiver geometries. We demonstrate the practicality of our model through case studies: 2D and 3D planar receivers. The accuracy of our formula is also validated by particle-based simulations. Advancing further, the explicit FAP density forms enable us to establish closed-form upper and lower bounds for the capacity of vertically-drifted FAP channels under a second-moment constraint, significantly advancing the understanding of FAP channels in MC systems.

==> 3Dcal.tex <==
\color{black} 
To derive the 3D FAP density for planar receivers, we consider a 3D It\^{o} diffusion $\mathbf{X}_t$ in $\R^3$ with a corresponding generator
$
A := \sum_{i=1}^3 v_i \dfrac{\partial}{\partial x_i} + \dfrac{\sigma^2}{2} \sum_{i=1}^3 \dfrac{\partial^2}{\partial x_i^2}
,
\label{e67}
$
where $v_i$ denotes the $i$-th component of the drift velocity $\mathbf{v}$.
We denote the Laplacian operator in 3D by $\Delta_3$ and consider the following BVP in Cartesian coordinate:
\begin{equation}
\left\{\begin{array}{ll}
A(\phi)=\sum_{i=1}^{3} v_{i} \frac{\partial \phi}{\partial x_{i}}+\frac{\sigma^2}{2} \Delta_3 \phi=0 & \text { in } \Omega \\
\phi=g & \text { on } \partial \Omega
\end{array}\right.
\label{e:BVP-2D}
,
\end{equation}
where $\phi$ is a (dummy) unknown function, $\Omega$ is the domain of \eqref{e:BVP-2D} defined by $\Omega=\mathbb{R}^{3} \cap\left\{x_{3}>0\right\}$, and $\partial\Omega$ is the boundary defined by $\partial\Omega=\mathbb{R}^{3} \cap\left\{x_{3}=0\right\}$. Here, we use the notation $x_j$ to indicate the $j$-th component of the position vector $\mathbf{x}=(x_1,\cdots,x_\text{D})$ in an $\text{D}$-dimensional space. We temporarily set $\sigma^2=1$.

\color{black}
To further simplify the calculation, we introduce a change of variable $\psi(\mathbf{x})=\gamma(\mathbf{x}) \phi(\mathbf{x})$, where
$
\gamma(\mathbf{x}):=\exp {\mathbf{v}^\tsp \mathbf{x}}=\exp \left(v_{1} x_{1}+v_{2} x_{2}+v_{3} x_{3}\right),
$
is the drift factor.
By this change of variable, we obtain a Helmholtz BVP:
\begin{equation}
\left\{\begin{array}{ll}
\tilde{A}(\psi)=\Delta_3 \psi-s^{2} \psi=0 & \text { in } \Omega \\
\psi=\tilde{g} & \text { on } \partial \Omega
\end{array}\right.
,
\label{BVP-3D2}
\end{equation}
where
$
s=\|\mathbf{v}\|
=\sqrt{v_1^2+v_2^2+v_3^2}
$
denotes the magnitude of the drift vector.
According to \cite{polyanin2001handbook}, the solution to equation \eqref{BVP-3D2} is given by
\begin{align}
\begin{split}
\psi(x_1,x_2,x_3)
=\int_{-\infty}^{\infty} \int_{-\infty}^{\infty} \tilde{g}(\xi,\eta)\left[\frac{\partial}{\partial \zeta} \tilde{G}(x_1,x_2,x_2,\xi,\eta,\zeta)\right]_{\zeta=0} d\xi d\eta,
\label{e:handbook2}
\end{split}
\end{align}
where the Green's function has the following form:
\begin{equation}
\begin{array}{c}
\tilde{G}(x_1, x_2, x_3, \xi, \eta, \zeta)=\dfrac{\exp \left(-s \mathcal{R}_{1}\right)}{4 \pi \mathcal{R}_{1}}-\dfrac{\exp \left(-s \mathcal{R}_{2}\right)}{4 \pi \mathcal{R}_{2}}, 
\end{array}
\label{e:handbook3}
\end{equation}
with
\begin{align}
\begin{split}
\mathcal{R}_1&:=\sqrt{(x_1-\xi)^{2}+(x_2-\eta)^{2}+(x_3-\zeta)^{2}},\\
\mathcal{R}_2&:=\sqrt{(x_1-\xi)^{2}+(x_2-\eta)^{2}+(x_3+\zeta)^{2}}
.
\label{e:handbook4}
\end{split}
\end{align}
%Detailed derivation of this Green's function can be found in \cite{tikhonov1990methods}.
We can write \eqref{e:handbook2} compactly as
\begin{equation}
\psi(\mathbf{x})=\int_{\mathbf{y}\in \partial \Omega}\left|\frac{\partial \tilde{G}(\mathbf{x}, \mathbf{y})}{\partial \mathbf{n}_\mathbf{y}}\right| \tilde{g}(\mathbf{y}) d \mathbf{y}.
\label{e:new-repre2D}
\end{equation}
From \eqref{e:handbook3}, we obtain the following explicit form by some simple calculus:
\begin{align}
\begin{split}
\left|\frac{\partial \tilde{G}(\mathbf{x}, \mathbf{y})}{\partial \mathbf{n}_{\mathbf{y}}}\right|
\Bigg\vert_{\partial \Omega}
=\frac{x_{3}}{2 \pi} \exp \{-s\|\mathbf{y}-\mathbf{x}\|\}\left\{\frac{1}{\|\mathbf{y}-\mathbf{x}\|^{3}}+\frac{s}{\|\mathbf{y}-\mathbf{x}\|^{2}}\right\} .
\label{e:calcul-00}
\end{split}
\end{align}


In order to obtain a representation formula for the solution $\phi$ of the original BVP \eqref{e:BVP-2D}, we substitute $\psi(\mathbf{x})=\gamma(\mathbf{x}) \phi(\mathbf{x})$ into \eqref{e:new-repre2D}, yielding
\begin{equation}
\begin{aligned}
\phi(\mathbf{x}) &= \frac{\psi(\mathbf{x})}{\gamma(\mathbf{x})} =\exp \{-\mathbf{v}^\tsp \mathbf{x}\} \int_{\partial \Omega}
\left|\frac{\partial \tilde{G}(\mathbf{x}, \mathbf{y})}{\partial \mathbf{n}_{\mathbf{y}}}\right| \tilde{g}(\mathbf{y}) d \mathbf{y} \\
&=\int_{\partial \Omega} \exp \left\{v_{1}\xi+v_{2}\eta-\mathbf{v}^\tsp \mathbf{x}\right\}
\left|\frac{\partial \tilde{G}(\mathbf{x}, \mathbf{y})}{\partial \mathbf{n}_{\mathbf{y}}}\right|
g(\mathbf{y}) d \mathbf{y} \\
&=\int_{\partial \Omega} \mathcal{K}_{\mathbf{v}}(\mathbf{x}, \mathbf{y}) g(\mathbf{y}) d \mathbf{y}
\end{aligned},
\label{e:calcul-01}
\end{equation}
where we used the relation between the boundary data: 
$
\tilde{g}(\mathbf{y})=e^{\mathbf{v}^{\mathsf{T}}\mathbf{y}}g(\mathbf{y})
$
and $\mathbf{y}=(\xi,\eta,0)$ on the boundary. We also use the notation $\mathcal{K}_{\mathbf{v}}(\mathbf{x}, \mathbf{y})$ to represent the overall integral kernel in the last equality of \eqref{e:calcul-01}.
%which is actually the partial derivative $\left|\frac{\partial G(\mathbf{x}, \mathbf{y})}{\partial \mathbf{n}_\mathbf{y}}\right|$, with Green's function $G$ corresponds to the original drift-diffusion BVP \eqref{e:BVP-2D}.

Next, we set $x_3=\lambda>0$, which is the vertical transmission distance.
Combining \eqref{e:calcul-00} and \eqref{e:calcul-01}, we obtain an exact formula for the integral kernel $\mathcal{K}_{\mathbf{v}}(\mathbf{x}, \mathbf{y})$:
\begin{equation}
\begin{aligned}
\mathcal{K}_\mathbf{v}(\mathbf{x},\mathbf{y})=&\ \exp \left\{v_{1} \xi+v_{2} \eta-\mathbf{v}^\tsp \mathbf{x}\right\}
\left|\frac{\partial \tilde{G}(\mathbf{x}, \mathbf{y})}{\partial \mathbf{n}_{\mathbf{y}}}\right|
\Bigg\vert_{\partial \Omega}
\\
=&\ \frac{\lambda}{2 \pi} \exp \{-\mathbf{v}^\tsp \mathbf{x}\} \exp \left\{v_{1} \xi+v_{2} \eta\right\}\cdot \exp \{-\|\mathbf{v}\|\|\mathbf{y}-\mathbf{x}\|\}\left[\frac{1}{\|\mathbf{y}-\mathbf{x}\|^{3}}+\frac{\|\mathbf{v}\|}{\|\mathbf{y}-\mathbf{x}\|^{2}}\right].
\end{aligned}
\end{equation}
This integral kernel can be interpreted as the probability density function of the FAP (see Section~\ref{section:generator}), so we denote it by $f_{\mathbf{Y} \mid \mathbf{X}}(\mathbf{y}|\mathbf{x})$ hereafter.

Lastly, to treat the general case $\sigma^2\neq 1$, we can simply replace $v_i$ with $\frac{v_i}{\sigma^2}$. This yields:
\begin{equation}
\begin{aligned}
f_{\mathbf{Y} \mid \mathbf{X}}(\mathbf{y}|\mathbf{x})
=\frac{\lambda}{2 \pi} \exp\left\{\left(\dfrac{\mathbf{v}}{\sigma^2}\right)^\tsp \left(\mathbf{y}-\mathbf{x}\right)\right\}\cdot \exp \left\{-\dfrac{\|\mathbf{v}\|}{\sigma^2}\norm{\mathbf{y}-\mathbf{x}}\right\}\left[\frac{1+\frac{\|\mathbf{v}\|}{\sigma^2}\norm{\mathbf{y}-\mathbf{x}}}{\norm{\mathbf{y}-\mathbf{x}}^{3}}\right],
\end{aligned}
\label{e:2Dresult}
\end{equation}
where $\mathbf{x}=(x_1,x_2,\lambda)$, $\mathbf{y}=(\xi,\eta,0)$, and $\lambda>0$ is the distance between the transmitter plane and the receiver plane.
Equation~\eqref{e:2Dresult} is the desired 3D FAP density function, allowing arbitrary drift directions.
\color{black}

==> old-section6.tex <==
\begin{comment}
\begin{figure}[ht]
    \centering
    \begin{subfigure}{\columnwidth} % Use \columnwidth to fit the subfigure within a single column
        \includegraphics[width=\linewidth]{Figures/Cap_Bound_vs_P.png}
        \caption{Caption for Subfigure 1}
        \label{fig:subfig1}
    \end{subfigure}

    \begin{subfigure}{\columnwidth} % Use \columnwidth to fit the subfigure within a single column
        \includegraphics[width=\linewidth]{Figures/Cap_Bound_vs_u.png}
        \caption{Caption for Subfigure 2}
        \label{fig:subfig2}
    \end{subfigure}
    \caption{Caption for the entire figure}
    \label{fig:main}
\end{figure}
\end{comment}
%%----
\subsection{Particle-based Verification of the Derived FAP Density Formulas}

\color{black}
For the 3D ($d=2$) scenario illustrated in Fig.~\ref{fig:dif-cha} where molecules are released from a point source at $[0,0,1]~\mu\mathrm{m}$ (so that the TX-RX distance $\lambda$ is $1~(\mu\mathrm{m})$), we conduct particle-based simulations (PBS) and numerical evaluations of theoretical FAP densities \eqref{e:2Dresult} for two different normalized drift vectors, one zero $\mathbf{u}=[0,0,0]$ and one non-zero $\mathbf{u}=[2,-3,-1]~(\mu\mathrm{m}^{-1})$. The resulting PDF of position deviation (which we called FAP noise) $[n_1,n_2]$ are shown in Fig.~\ref{fig:planarRX_both} and Fig.~\ref{fig:planarRX_drift_both}, respectively. 

For PBS, we adopt the 
%Euler-Maruyama discretization of Brownian motion with drift 
the Monte Carlo method \cite[Eq. (9)-(11)]{farsad2016comprehensive} to simulate $M=10^6$ independent trajectories of dissolved Ethanol molecules diffusing in water (with a diffusion coefficient $D$ of roughly $840~(\mu\mathrm{m}^2/\mathrm{sec})$) with a time step of $10^{-6}(\mathrm{sec})$. The first hitting position of a molecule is approximated by taking the first two coordinates after the third coordinate value first becomes negative (i.e., first crosses the receiver plane $x_3=0$). The resulting FAP density estimates are given in Fig.~\ref{fig:planarRX_particle} and Fig.~\ref{fig:planarRX_drift_particle}, respectively. For theoretical predictions, we compute the derived FAP density formula \eqref{e:2Dresult}. While producing these figures, we truncate values lower than $10^{-3}$ to highlight the approximate support of the distribution (notice that in theory, the support of FAP distributions is all of $\mathbb{R}^2$, i.e., the particle might arrive anywhere on the whole planar receiver). 

For the no-drift scenario, our PBS result (Fig.~\ref{fig:planarRX_particle}) reveals a symmetrical distribution of particles around the origin, consistent with the predictions of our derived density function (Fig.~\ref{fig:planarRX_numerical}). In the presence of a drift vector, the particle distribution 
tilts towards the direction of parallel normalized drift $\mathbf{u}_\text{par}=[2,-3]~(\mu\mathrm{m}^{-1})$ (see Fig.~\ref{fig:planarRX_drift_particle}), aligning with our theoretical expectations (Fig.~\ref{fig:planarRX_drift_numerical}).

As shown in Fig.~\ref{fig:planarRX_both} and Fig.~\ref{fig:planarRX_drift_both}, our theoretical prediction matches well with particle-based simulation results, noticing that the error in the density estimate via particle-based simulations is on the order of $1/\sqrt{M}=10^{-3}$. Therefore, the PBS and numerical evaluation of the theoretical formula provide strong evidence supporting the accuracy and reliability of our derived FAP density function. They demonstrate not only the validity of our model under different conditions but also its robustness in predicting particle behavior in molecular communication systems.

\color{black}

\begin{figure}[ht]
    \centering
    \begin{subfigure}{\columnwidth} % Use \columnwidth to fit the subfigure within a single column
        \includegraphics[width=\linewidth]{Figures/pbs_lambda1_u000_notitle.eps}
        \caption{Particle-based simulated FAP density on a planar receiver when drift is zero.}
        \label{fig:planarRX_particle}
    \end{subfigure}

    \begin{subfigure}{\columnwidth} % Use \columnwidth to fit the subfigure within a single column
        \includegraphics[width=\linewidth]{Figures/pdf_lambda1_u000_notitle.eps}
        \caption{Theoretical FAP density \eqref{e:2Dresult} on a planar receiver when drift is zero.}
        \label{fig:planarRX_numerical}
    \end{subfigure}
    \caption{Comparison of theoretical and simulated FAP densities on a planar receiver (i.e., $d=2$) for zero drift $\mathbf{u}=[0,0,0]$.}
    \label{fig:planarRX_both}
\end{figure}

\begin{figure}[ht]
    \centering
    \begin{subfigure}{\columnwidth} % Use \columnwidth to fit the subfigure within a single column
        \includegraphics[width=\linewidth]{Figures/pbs_lambda1_u2-3-1_notitle.eps}
        \caption{Particle-based simulated FAP density on a planar receiver when normalized drift $\mathbf{u}$ is $[2, -3, -1]$ $(\mu \text{m}^{-1})$.}
        \label{fig:planarRX_drift_particle}
    \end{subfigure}

    \begin{subfigure}{\columnwidth} % Use \columnwidth to fit the subfigure within a single column
        \includegraphics[width=\linewidth]{Figures/pdf_lambda1_u2-3-1_notitle.eps}
        \caption{Theoretical FAP density \eqref{e:2Dresult} on the planar receiver when normalized drift $\mathbf{u}$ is $[2, -3, -1]$ $(\mu \text{m}^{-1})$.}
         \label{fig:planarRX_drift_numerical}
    \end{subfigure}
    \caption{Comparison of theoretical and simulated FAP densities on a planar receiver (i.e., $d=2$) for a case of non-zero normalized drift $\mathbf{u}=[2,-3,-1]~(\mu\mathrm{m}^{-1})$.}
    \label{fig:planarRX_drift_both}
\end{figure}
%%----
\color{red}
\subsection{Graphical Illustration of Trends of Capacity Bounds}
\color{black}

\begin{comment}
Version 1:

\color{olive}
Thank you for your valuable suggestion regarding the illustration of capacity bounds. In light of your feedback, we have included numerical evaluations (Figure~2) that demonstrate the impact of key parameters on the capacity bounds in the context of a 3D scenario (where \( D = 3 \) and thus \( d = 2 \)), as formulated in Eqs.~(46) and (39) of the manuscript.

In Figure~\ref{fig:cap-P}, we explore how capacity increases with the transmission power (\( P \)). Figure~\ref{fig:cap-lambda} illustrates the inverse relationship between capacity and the separation distance (\( \lambda \)) between the transmitter and receiver. Crucially, Figure~\ref{fig:cap-u} highlights the effect of normalized drift (\( u \)), which represents flow velocity, on the capacity. This figure provides insight into the comprehensiveness and tightness of the bounds, particularly emphasizing how the upper and lower bounds diverge or converge under varying flow velocities. This analysis offers a clearer understanding of the bounds' behavior and their practical implications in a 3D planar receiver context.
\color{black}
\end{comment}

\color{black}
In this subsection, we have included numerical evaluations to demonstrate the impact of key factors on the capacity bounds as derived in Eqs.~(46) and (39) for a two-dimensional scenario (\( d=2 \)). In Figure~\ref{fig:cap-P}, we illustrate how capacity increases with the transmission power (\( P \)). Figure~\ref{fig:cap-lambda} shows the inverse relationship between capacity and the distance between the transmitter and receiver (\( \lambda \)). Furthermore, Figure~\ref{fig:cap-u} depicts the effect of normalized drift (\( u \)) on capacity, particularly noting the reduced effectiveness of the upper bound as \( u \) approaches zero.

These figures provide insight into the comprehensiveness and tightness of the bounds, particularly emphasizing how the upper and lower bounds diverge or converge under various key parameters.
\color{black}


\begin{comment}
\begin{figure}[ht]
    \centering
    \begin{subfigure}{\columnwidth} % Use \columnwidth to fit the subfigure within a single column
        \includegraphics[width=\linewidth]{Figures/Cap_Bound_vs_P.png}
        \caption{Caption for Subfigure 1}
        \label{fig:subfig1}
    \end{subfigure}

    \begin{subfigure}{\columnwidth} % Use \columnwidth to fit the subfigure within a single column
        \includegraphics[width=\linewidth]{Figures/Cap_Bound_vs_u.png}
        \caption{Caption for Subfigure 2}
        \label{fig:subfig2}
    \end{subfigure}
    \caption{Caption for the entire figure}
    \label{fig:main}
\end{figure}
\end{comment}
%%
\begin{figure}
    \centering
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Cap_Bound_vs_P_notitle.eps}
        \caption{Capacity bounds versus second-moment constraint \( P \) with $\lambda=1~(\mu\mathrm
        {m})$ and $u=-1~(\mu\mathrm{m}^{-1})$ fixed.}
        \label{fig:cap-P}
    \end{subfigure}
    \hfill
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Cap_Bound_vs_lambda_notitle.eps}
        \caption{Capacity bounds versus TX-RX distance \( \lambda \) with $P=1~(\mu\mathrm
        {m}^2)$ and $u=-1~(\mu\mathrm{m}^{-1})$ fixed.}
        \label{fig:cap-lambda}
    \end{subfigure}
    \hfill
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Cap_Bound_vs_u_notitle.eps}
        \caption{Capacity bounds versus absolute normalized drift \( |u| \) with $P=1~(\mu\mathrm
        {m}^2)$ and $\lambda=1~(\mu\mathrm
        {m})$ fixed.}
        \label{fig:cap-u}
    \end{subfigure}
    \caption{Numerical evaluations of derived capacity bounds for \( d=2 \), illustrating the influence of \( P \), \( \lambda \), and \( u \) on the trends of capacity.}
    \label{fig:three-graphs}
\end{figure}
%%

==> old-section7.tex <==
\textcolor{red}{(Need to Rewrite)}

In this paper, we explored two fundamental problems in the field of diffusive \textcolor{blue}{MC}: characterization of the first arrival position (FAP) density and the capacity bounding problem of vertically-drifted FAP channels.

We first presented a unified approach to the FAP density characterization problem for MC systems with a fully-absorbing receiver. Our approach establishes a connection between (macroscopic) partial differential equation models and (microscopic) stochastic differential equation models.
Using stochastic analysis tools, we proposed a concise expression, represented by \eqref{eq:main}, which relates the FAP density to the elliptic-type Green's function. Notably, this expression is applicable to any spatial dimension, drift direction, and receiver shape.


In addition, we demonstrated 
(in Appendix~\ref{sec:case})
the effectiveness of our approach by providing special case calculations: the 2D linear receiver, the 3D planar receiver, and the 3D spherical receiver. We showed that our approach can precisely reproduce known results on FAP density in the literature. Moreover, for the 2D linear receiver case, our approach improves upon the existing formula by accommodating arbitrary drift directions.

Having access to the explicit forms of FAP density, we are able to conduct a more comprehensive analysis of the proposed MC system, which utilizes position information. In particular, 
we addressed the problem of bounding the capacity
of vertically-drifted FAP channels under the covariance (matrix) constraint.

Drawing inspiration from vector Gaussian interference channels, we provided closed-form upper and lower bounds on this capacity in the three-dimensional setting. This was achieved through a detailed analysis of the characteristic function of vertically-drifted FAP noise distributions, which also led to the discovery of a novel weak stability property intrinsic to vertically-drifted FAP noise distributions.

Our findings contribute to the ongoing efforts to comprehend the fundamental limits of \textcolor{blue}{MC} systems. They also open new avenues for future research, including extending the analysis to other spatial dimensions, exploring the implications of the discovered weak stability property, and investigating other settings beyond the vertically-drifted case.


==> oldmethod.tex <==
For the sake of completeness, we review in a self-contained fashion the old approach to finding FAP density function in previous work
such as \cite{pandey2018molecular}. Throughout this section, we set the $x$-direction to be the direction of transmission, i.e. the direction pointing from Tx to Rx.

\subsection{Finding the Green's Function in Free Space}
For a 2-dimensional (2D) diffusion channel with a constant drift velocity $\mathbf{v}=(v,0)$ pointing from the transmitter to the receiver along the $x$-axis, equation \eqref{ad-eq} can be written explicitly as
\begin{equation}
\frac{\partial c(x, y, t)}{\partial t}+v \frac{\partial c(x, y, t)}{\partial x}=D\left(\frac{\partial^{2} c(x, y, t)}{\partial x^{2}}+\frac{\partial^{2} c(x, y, t)}{\partial y^{2}}\right)
\label{2d-ad-eq}
\end{equation}
where $c(x, y, 0)=\delta\left(x-x_{0}\right) \delta\left(y-y_{0}\right)$ is the 2D Dirac delta function. The boundary condition is set to be: 
\begin{equation}
c(x,y,t)=0
\quad\text{for}\quad
x, y \in \partial\Omega,
\label{2d-ad-eq-bd}
\end{equation}
representing an absorbing receiver.

Using separation of variables, the concentration field $c(x,y,t)$ can be written as 
\begin{equation}
c(x,y,t)=c_1(x,t)c_2(y,t)
.
\label{eq:separate}
\end{equation}
By plugging \eqref{eq:separate} back into \eqref{2d-ad-eq}, we get two separated equations
\begin{align}
\frac{\partial c_{1}}{\partial t}+v \frac{\partial c_{1}}{\partial x}-D \frac{\partial^{2} c_{1}}{\partial x^{2}}&=0,
\label{eq:s1}
\\ \frac{\partial c_{2}}{\partial t}-D \frac{\partial^{2} c_{2}}{\partial y^{2}}&=0.
\label{eq:s2}
\end{align}
The \textit{fundamental solutions} (aka free space Green's function) of \eqref{eq:s1} and \eqref{eq:s2} are
\begin{equation}
c_{1}(x, t)=\frac{1}{\sqrt{4 \pi D t}} \exp \left(-\frac{\left(x-x_{0}-v t\right)^{2}}{4 D t}\right)
\label{eq:s3}
\end{equation}
and
\begin{equation}
c_{2}(y, t)=\frac{1}{\sqrt{4 \pi D t}} \exp \left(-\frac{\left(y-y_{0}\right)^{2}}{4 D t}\right)
\label{eq:s4}
\end{equation}
respectively.
Hence, the free space Green's function of \eqref{2d-ad-eq} can be written as the product of \eqref{eq:s3} and \eqref{eq:s4}:
\begin{align}
\begin{split}
&G\left(x, y, x_{0}, y_{0}, t\right)\\
=\ &\frac{1}{4 \pi D t} \exp \left(\frac{-\left(x-x_{0}-v t\right)^{2}-\left(y-y_{0}\right)^{2}}{4 D t}\right).
\end{split}
\label{eq:s5}
\end{align}

\subsection{Finding the Green's Function for Absorbing Boundary Condition}
For \eqref{eq:s5}, we have not yet taken the boundary conditions into account. Since the receiver is assume to be perfectly absorbing, we require the concentration to be zero on the boundary, as \eqref{2d-ad-eq-bd} shows.

There is one well-known method, originated in classical electrodynamics, that works well in problems of finding static distributions for flat boundaries, called \textit{the method of image}, see \cite{jackson1999classical}.
Since we only care about the concentration function inside the domain, we can effectively put an ``mirror image'' of negative mass at the reflection point of the original releasing point. Using this method, the domain of the original unknown function is not extended, but the function is made to satisfy given boundary conditions, such as absorbing boundary in our case. 

To use the method of image, we write
\begin{align}
\begin{split}
&G_{\text{abs}}(x,y,x_0,y_0,t)\\
=\ &G(x,y,x_0,y_0,t)-a(x_0)G(x,y,-x_0,y_0,t)
\end{split}
\end{align}
and then solve for $a(x_0)$. Note that the subscript ``abs'' stands for absorbing. The absorbing boundary condition requires that
\begin{equation}
a(x_0) 
= \dfrac{G(0,y,x_0,y_0,t)}{G(0,y,-x_0,y_0,t)}
=\exp\left(-\dfrac{x_0 v}{D}\right)
.\label{compensate-term}
\end{equation}
We can now write down the Green's function for absorbing boundary as
\begin{equation}
\begin{aligned}
&G_{\text{abs}}\left(x, y, x_{0}, y_{0}, t\right)\\
=\ & \frac{1}{4 \pi D t}\left[\exp \left(-\frac{\left(x-x_{0}-v t\right)^{2}+\left(y-y_{0}\right)^{2}}{4 D t}\right)\right]\\
&\left.-\exp \left(-\frac{x_{0} v}{D}-\frac{\left(x+x_{0}-v t\right)^{2}+\left(y-y_{0}\right)^{2}}{4 D t}\right)\right]
\end{aligned}
.
\label{green-abs}
\end{equation}
\subsection{From Green's function to FAP Density}
Consider a quantity called \textit{diffusive flux} $J(0,y,t)$ at $x=0$ plane, which possesses a physical unit of particle density per unit length per unit time. By Fick's law, we know that 
\begin{equation}
J(0,y,t)
= -D\dfrac{\partial G_{\text{abs}}(x,y,x_0,y_0,t)}{\partial x}
.\end{equation}
Using the absorbing Green's function formula as shown in \eqref{green-abs}, we can calculate the flux explicitly, yielding
\begin{equation}
J(0,y,t)=-\frac{x_0}{4 \pi D t^2} \exp \left(-\frac{\left(x_{0}+v t\right)^{2}+\left(y-y_{0}\right)^{2}}{4 D t}\right)
.
\label{eq:55}
\end{equation}
Note that the original formula \cite[Eq.~(14)] {pandey2018molecular} has some calculation error, so we correct the formula herein.

Our goal is to find the FAP density $f(\mathbf{y}|\mathbf{x})$. Let $\mathbf{x}=\left(x_{0}, y_{0}\right)$ denote the point of release of the information molecule and $\mathbf{y}=(x, y)$ its arrival position at the receiver boundary. The conditional PDF of $Y$ at a receiver located at $x=0$ is given as
\begin{equation}
f_{Y \mid X}(0,y \mid x_0,y_0)=\left.\int_{0}^{\infty} J(0, y, t) \mathrm{d} t\right
..
\label{eq:56}
\end{equation}
Plugging the diffusion flux we just obtained in \eqref{eq:55} into \eqref{eq:56}, we have
\begin{align}
\begin{split}
&f_{Y \mid X}(0,y \mid x_0,y_0)\\
=\ &-\int_{0}^{\infty} \frac{x_0}{4 \pi D t^2} \exp \left(-\frac{\left(x_{0}+v t\right)^{2}+\left(y-y_{0}\right)^{2}}{4 D t}\right) \mathrm{d} t
.
\end{split}
\end{align}
In order to calculate this integration explicitly, we rearrange the terms to get
\begin{align}
\begin{split} 
&f_{Y \mid X}(0,y \mid x_0,y_0)\\
=\ &\ \frac{-x_0}{4 \pi D} \exp \left(-\frac{x_{0} v}{2 D}\right) \\ & \times \int_{0}^{\infty} \frac{1}{t^2} \exp \left(-\frac{x_{0}^{2}+\left(y-y_{0}\right)^{2}}{4 D t}-\frac{v^{2} t}{4 D}\right) \mathrm{d} t. 
\end{split}
\label{1-eq17}
\end{align}
Letting $K_{s}(z)$ be the modified Bessel function of the second kind of order $s$, for positive constants $a$ and $b$, we have the relation \cite{gradshteyn1988tables}:
\begin{equation}
\int_{0} t^{-s-1} \exp \left(-\left(\frac{a}{t}+b t\right)\right) \mathrm{d} t=2\left(\frac{b}{a}\right)^{s / 2} K_{s}(2 \sqrt{a b})
,
\label{1-eq18}
\end{equation}
where $s$ and $z$ are real and complex numbers respectively. 
Combining \eqref{1-eq17} and \eqref{1-eq18} with $x_{0}=d$, we finally get
\begin{align}
\begin{split}
&f(\mathbf{y}|\mathbf{x})\\
=\ &f_{Y \mid X}(0,y \mid d,y_0)\\
=\ &\frac{|v|d}{2 \pi D} \exp \left(\frac{-d v}{2 D}\right) 
\dfrac{1}{\sqrt{\left(d^{2}+\left(y-y_0\right)^{2}\right)}}\\
&\cdot K_1\left(\frac{|v|\sqrt{\left(d^{2}+\left(y-y_{0}\right)^{2}\right)}}{2 D}\right).
\end{split}
\label{eq71}
\end{align}
It is worth noting that the conditional FAP density as shown in
\eqref{eq71} depends only on $y-y_{0}$, but not on time variable $t$. We can conclude that the FAP channel is an additive time-invariant channel.


==> preli.tex <==
\subsection{Capacity for Gaussian Channel}
\label{sec:pre-A}
We briefly review some background knowledge about mutual information and channel capacity for later use.
Let $X$ be a random variable with a probability density function $f$ whose support is denoted by $\mathcal{X}$.
The (differential) entropy $h(X)$ is defined as: 
\begin{equation}
h(X):=\E_X[-\ln f(X)]=-\int_{\mathcal{X}}  [\ln f(x)] f(x)dx.
\end{equation}
Based on the definition of entropy, the mutual information between the input and output of the additive channel 
\begin{equation}
    Y=X+N
\end{equation}
is given by
\begin{align}
    I(X;Y) &= h(Y) - h(Y|X)\\
    &=h(Y) - h(X+N|X)\\
    &=h(Y) - h(X|X) - h(N|X)\\
    &=h(Y) - h(N).
\end{align}
Here we have assumed that the noise $N$ is independent of signal $X$.
Recall that the (Shannon) channel capacity is defined as:
\begin{equation}
C = \sup_{f_X(x)} I(X;Y).
\label{eq:inpc}
\end{equation}
The supremum is taken over all possible distributions of $X$ satisfying some chosen constraint. For point-to-point communication or single-input-single-output (SISO) scenarios, sometimes the output constraints are used instead of the input constraints, yielding
\begin{equation}
C = \sup_{f_Y(x)} I(X;Y).
\label{eq:outpc}
\end{equation}

The selection of constraint depends heavily on the noise distribution. To get some feeling about this, let us study a simple example before exploring the FAP channels. For additive Gaussian channel (i.e. the noise is Gaussian distributed), the most familiar power measure is the second moment constraint. We can prescribe our signal set to satisfy:
\begin{equation}
    \E[X^2] 
    = \int_{\mathcal{X}} x^2 f(x)dx \leq P.
\label{eq:2pc}
\end{equation}
The constant $P\geq 0$ is the maximum power we allowed for all input signals.
Using this power constraint \eqref{eq:2pc}, the channel capacity \eqref{eq:inpc} can be written as:
\begin{equation}
C = \sup_{f_X(x) :\  \E[X^2]\leq P} I(X;Y).  \end{equation}
Following a standard textbook derivation (see \cite{cover1999elements}), one can see that the supremum value of $I(X;Y)$ is
\begin{equation}
\frac{1}{2}\ln\left(\frac{\sigma^2+P}{\sigma^2}\right), 
\label{eq:13}
\end{equation}
and the capacity attaining distribution is normal distributed with variance $P$, namely, $X \sim \mathcal{N}(0,P)$.

In order to compare to the capacity formula of FAP channels, we let $A^2:=\sigma^2+P$ and rewrite \eqref{eq:13} in the following way:
\begin{align}
\begin{split}
C_{\text{G}}
=C(A,\sigma)
=\frac{1}{2}\ln\left(\dfrac{A^2}{\sigma^2}\right)
=\ln\left(\dfrac{A}{\sigma}\right),
\end{split}
\end{align}
where the subscript $\text{G}$ stands for Gaussian.

\subsection{Density Function and Entropy of Multivariate Cauchy Distributions}\label{sec:pre-B}
The Cauchy distribution, named after Augustin Cauchy, is a continuous probability distribution often used in statistics as a canonical example of distribution since both its expected value and its variance are undefined. It is also known, especially among physicists, as the Lorentz distribution.
In mathematics, it is closely related to the fundamental solution for the Laplace equation in the half-plane, and it is one of the few distributions that is stable (see \cite{pierce1997application,fahs2012capacity}) and has a density function that can be expressed analytically. (Other examples are normal distribution and L\'{e}vy distribution.)

The univariate\footnote{For univariate Cauchy, people usually suppress the word ``univariate'', and simply call it Cauchy.} Cauchy distribution has the probability density function (PDF) which can be expressed as:
\begin{equation}
    f(x;x_0,\gamma) =
    \dfrac{1}{\pi \gamma} 
    \dfrac{\gamma^2}
    {(x-x_0)^2+\gamma^2
    }
    =
    \dfrac{1}{\pi \gamma} 
    \dfrac{1}
    {1+(\frac{x-x_0}{\gamma})^2
    },
\label{eq:ch-dist}
\end{equation}
where $x_0\in \mathbb{R}$ is the location parameter, and $\gamma>0$ is the scaling parameter (see \cite{shao1993signal}). 
For the purpose of exploring the channel capacity, since the location parameter $x_0$ is irrelevant to the entropy, we may assume without loss of generality that $x_0=0$, yielding
the so called \textit{symmetry Cauchy} with PDF as:
\begin{equation}
    f(x;\gamma) =
    \dfrac{\gamma}{\pi} 
    \dfrac{1}
    {x^2+\gamma^2
    }
    =
    \dfrac{1}{\pi \gamma} 
    \dfrac{1}
    {1+(\frac{x}{\gamma})^2
    }.
\label{eq:sm-ch-dist}
\end{equation}
The entropy of Cauchy distribution can be evaluated by direct calculation. From \eqref{eq:ch-dist}, we have
\begin{equation}
    h(X)=\ln(4\pi \gamma)
\end{equation}
whenever $X\sim \rm{Cauchy}(x_0,\gamma)$, and $x_0$ can be chosen arbitrarily.


As for multivariate Cauchy distribution, our notation system mainly follows \cite{kotz2004multivariate}.
Consider a $p$-dimensional Euclidean random vector $\mathbf{X}=(X_1,\cdots,X_p)^\top$ which follows multivariate Cauchy distribution.
We use the notation $\mathbf{X} \sim {\rm Cauchy}_p(\boldsymbol\mu,\Sigma)$ to specify the parameters, where $\boldsymbol\mu\in\R^{p\times 1}$ is the location vector, and $\Sigma\in\R^{p\times p}$ is the scale matrix describing the shape of the distribution.
The PDF of multivariate Cauchy distribution is given by
the following formula:
\begin{align}
\begin{split}
    &f_{\mathbf{X}}^{(p)}(\mathbf{x};\boldsymbol\mu,\Sigma)\\
    =&\ \dfrac{\Gamma(\frac{1+p}{2})}
    {\Gamma(\frac{1}{2})\pi^{\frac{p}{2}}
    |\Sigma|^{\frac{1}{2}}
    [1+(\mathbf{x}-\boldsymbol\mu)^\top\Sigma^{-1}(\mathbf{x}-\boldsymbol\mu)]^\frac{1+p}{2}
    }.
\end{split}    
\label{eq:pvariate-ch-dist}
\end{align}
Note that $\Sigma$ is by nature a positive-definite square matrix.
For our later purpose, we mainly work in the case $p=2$. We provide the PDF of this special case here for convenience:
\begin{align}
\begin{split}
    &f_{\mathbf{X}}^{(2)}(\mathbf{x};\boldsymbol\mu,\Sigma)\\
    =&\ \dfrac{\Gamma(\frac{3}{2})}
    {\pi^{\frac{3}{2}}
    |\Sigma|^{\frac{1}{2}}
    [1+(\mathbf{x}-\boldsymbol\mu)^\top\Sigma^{-1}(\mathbf{x}-\boldsymbol\mu)]^\frac{3}{2}
    }.
\end{split}
\label{eq:bivariate-ch-dist}
\end{align}
Equation~\eqref{eq:bivariate-ch-dist} is the so-called bivariate Cauchy distribution.

Similar to the univariate case,
we can without loss of generality set $\boldsymbol\mu=\mathbf{0}$ in \eqref{eq:pvariate-ch-dist} and \eqref{eq:bivariate-ch-dist} for the purpose of entropy and channel capacity analysis.
When $\boldsymbol\mu = \mathbf{0}$, the multivariate Cauchy is called \textit{central}. For the case that the Cauchy is central, we abuse the notations ${\rm R}$ and $\Sigma$ to mean the same scale matrix.
We shall assume all Cauchy distributions considered in this paper to be central from now on. In addition, for the special case that $\Sigma$ is a diagonal matrix, 
namely
\begin{equation}
\Sigma=\text{diag}(\gamma^2,\gamma^2)
=\begin{bmatrix}
\gamma^2&0\\
0&\gamma^2
\end{bmatrix},
\end{equation}
the central bivariate Cauchy density function can be simplified into a more concise form:
\begin{equation}
\dfrac{1}{2\pi}
\dfrac{\gamma}{
(n_1^2+n_2^2+\gamma^2)^{3/2}
},
\label{eq:simple-bi-ch}
\end{equation}
where $\mathbf{n}=(n_1,n_2)$ is the Cauchy random vector.

Finally, the (differential) entropy of $p$-variate central Cauchy distribution can be found in [4]. We briefly state the results here for later use. Suppose the scale matrix ${\rm R}$ of a $p$-variate Cauchy $\mathbf{X}$ is prescribed, the entropy of $\mathbf{X}$ can be expressed as
\begin{equation}
    h(\mathbf{X};{\rm R})=\dfrac{1}{2}\ln|{\rm R}|+\Phi(p),
\end{equation}
where $|{\rm R}|$ represents the determinant of matrix ${\rm R}$; $\Phi(p)$ is a constant depending only on dimension $p$, and it can be evaluated through
\begin{align}
\begin{split}
    \Phi(p)
    =&\ \ln
    \left[
    \dfrac{\pi^{\frac{p}{2}}}{\Gamma(\frac{p}{2})}B\left(\frac{p}{2},\dfrac{1}{2}\right)
    \right]\\
    &\quad +\dfrac{1+p}{2}\left[
    \psi\left(\frac{1+p}{2}\right)-\psi\left(\frac12\right)
    \right].
\end{split}
\end{align}
In the above expression, $B(x,y)=\frac{\Gamma(x)\Gamma(y)}{\Gamma(x+y)}$ is the so-called \textit{beta function}, and
\begin{equation}
\psi(t):=\dfrac{d}{dt}\big[\ln\Gamma(t)\big]   
\end{equation}
is known as the \textit{digamma function}.


